Beam Search for Error-Correcting Codes via Conditional Diffusion

We introduce a diffusion framework for neural decoding of error-correcting codes (ECCs). We interpret decoding as a conditional diffusion process that progressively predicts codeword bits while treating the physical channel observation as fixed side information. At each stage, a neural model estimates bitwise posteriors conditioned on the physical observation and the current noisy state of the codeword. We focus particularly on masked diffusion, for which the reverse process naturally induces a Maxwell beam search (MBS) procedure inspired by the Maxwell construction of Measson et al. Rather than committing to a single uncertain decision, the decoder maintains multiple candidate trajectories, removes parity-infeasible candidates, and ranks the remaining candidates using accumulated reverse-transition log-probabilities. We evaluate the framework across multiple code families on binary phase-shift keying (BPSK) over additive white Gaussian noise (AWGN). Experiments show competitive decoding performance across Polar, low-density parity-check (LDPC), and Bose-Chaudhuri-Hocquenghem (BCH) codes. The MBS decoder consistently improves upon the corresponding single-trajectory diffusion decoder and, in all evaluated settings, improves upon available neural decoding results.

==> figures/data/ccsds-stopping-histograms.tex <==
% Generated by figures/data/build-stopping-time.py; do not edit counts by hand.
\nextgroupplot[]
\definecolor{histcolor}{HTML}{0072B2}
\node[anchor=south,font=\scriptsize\bfseries,text=histcolor,inner sep=0pt,yshift=6pt] at (rel axis cs:0.5,1) {\ifdefined\arxivlayout\shortstack{\mbsresult{2048}\\2.5 dB}\else\strut \revision2{MBS}, 2.5 dB\fi};
\path[draw=none,fill=histcolor!85] (axis cs:0.1,0.00007) rectangle (axis cs:1.9,0.66);
\path[draw=none,fill=histcolor!85] (axis cs:11.1,0.00007) rectangle (axis cs:12.9,0.264);
\path[draw=none,fill=histcolor!85] (axis cs:12.1,0.00007) rectangle (axis cs:13.9,0.031);
\path[draw=none,fill=histcolor!85] (axis cs:18.1,0.00007) rectangle (axis cs:19.9,0.012);
\path[draw=none,fill=histcolor!85] (axis cs:19.1,0.00007) rectangle (axis cs:20.9,0.005);
\path[draw=none,fill=histcolor!85] (axis cs:20.1,0.00007) rectangle (axis cs:21.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:25.1,0.00007) rectangle (axis cs:26.9,0.003);
\path[draw=none,fill=histcolor!85] (axis cs:26.1,0.00007) rectangle (axis cs:27.9,0.002);
\path[draw=none,fill=histcolor!85] (axis cs:27.1,0.00007) rectangle (axis cs:28.9,0.002);
\path[draw=none,fill=histcolor!85] (axis cs:32.1,0.00007) rectangle (axis cs:33.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:33.1,0.00007) rectangle (axis cs:34.9,0.002);
\path[draw=none,fill=histcolor!85] (axis cs:39.1,0.00007) rectangle (axis cs:40.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:40.1,0.00007) rectangle (axis cs:41.9,0.002);
\path[draw=none,fill=histcolor!85] (axis cs:41.1,0.00007) rectangle (axis cs:42.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:42.1,0.00007) rectangle (axis cs:43.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:47.1,0.00007) rectangle (axis cs:48.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:48.1,0.00007) rectangle (axis cs:49.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:49.1,0.00007) rectangle (axis cs:50.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:54.1,0.00007) rectangle (axis cs:55.9,0.002);
\path[draw=none,fill=histcolor!85] (axis cs:55.1,0.00007) rectangle (axis cs:56.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:56.1,0.00007) rectangle (axis cs:57.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:64.1,0.00007) rectangle (axis cs:65.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:78.1,0.00007) rectangle (axis cs:79.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:92.1,0.00007) rectangle (axis cs:93.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:95.1,0.00007) rectangle (axis cs:96.9,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:96.1,0.00007) rectangle (axis cs:97.9,0.001);
\node[anchor=west,font=\scriptsize,text=histcolor,inner sep=1pt] at (axis cs:4,0.66) {66\%};
\node[anchor=south east,font=\scriptsize,text=histcolor,inner sep=1pt,yshift=2pt] at (axis cs:97,0.001) {0.1\%};
\nextgroupplot[yticklabels={},xmax=10,xtick={0,2,4,6,8,10},xticklabels={0,2,4,6,8,10}]
\definecolor{histcolor}{HTML}{D55E00}
\node[anchor=south,font=\scriptsize\bfseries,text=histcolor,inner sep=0pt,yshift=6pt] at (rel axis cs:0.5,1) {\strut SB-ECC, 2.5 dB};
\path[draw=none,fill=histcolor!85] (axis cs:1.68,0.00007) rectangle (axis cs:2.32,0.001);
\path[draw=none,fill=histcolor!85] (axis cs:2.68,0.00007) rectangle (axis cs:3.32,0.013);
\path[draw=none,fill=histcolor!85] (axis cs:3.68,0.00007) rectangle (axis cs:4.32,0.127);
\path[draw=none,fill=histcolor!85] (axis cs:4.68,0.00007) rectangle (axis cs:5.32,0.27);
\path[draw=none,fill=histcolor!85] (axis cs:5.68,0.00007) rectangle (axis cs:6.32,0.278);
\path[draw=none,fill=histcolor!85] (axis cs:6.68,0.00007) rectangle (axis cs:7.32,0.129);
\path[draw=none,fill=histcolor!85] (axis cs:7.68,0.00007) rectangle (axis cs:8.32,0.039);
\path[draw=none,fill=histcolor!85] (axis cs:8.68,0.00007) rectangle (axis cs:9.32,0.143);
\node[anchor=south,font=\scriptsize,text=histcolor,inner sep=1pt,yshift=2pt] at (axis cs:6,0.278) {27.8\%};
\node[anchor=south east,font=\scriptsize,text=histcolor,inner sep=1pt,yshift=2pt] at (axis cs:2,0.001) {0.1\%};
\nextgroupplot[yticklabels={}]
\definecolor{histcolor}{HTML}{0072B2}
\node[anchor=south,font=\scriptsize\bfseries,text=histcolor,inner sep=0pt,yshift=6pt] at (rel axis cs:0.5,1) {\ifdefined\arxivlayout\shortstack{\mbsresult{64}\\4 dB}\else\strut \revision2{MBS}, 4 dB\fi};
\path[draw=none,fill=histcolor!85] (axis cs:0.1,0.00007) rectangle (axis cs:1.9,0.985539);
\path[draw=none,fill=histcolor!85] (axis cs:11.1,0.00007) rectangle (axis cs:12.9,0.0131592);
\path[draw=none,fill=histcolor!85] (axis cs:12.1,0.00007) rectangle (axis cs:13.9,0.00115685);
\path[draw=none,fill=histcolor!85] (axis cs:25.1,0.00007) rectangle (axis cs:26.9,0.000144606);
\node[anchor=west,font=\scriptsize,text=histcolor,inner sep=1pt] at (axis cs:4,0.985539) {98.6\%};
\node[anchor=south west,font=\scriptsize,text=histcolor,inner sep=1pt,yshift=2pt] at (axis cs:26,0.000144606) {0.0145\%};
\nextgroupplot[yticklabels={},xmax=10,xtick={0,2,4,6,8,10},xticklabels={0,2,4,6,8,10}]
\definecolor{histcolor}{HTML}{D55E00}
\node[anchor=south,font=\scriptsize\bfseries,text=histcolor,inner sep=0pt,yshift=6pt] at (rel axis cs:0.5,1) {\strut SB-ECC, 4 dB};
\path[draw=none,fill=histcolor!85] (axis cs:0.68,0.00007) rectangle (axis cs:1.32,0.01);
\path[draw=none,fill=histcolor!85] (axis cs:1.68,0.00007) rectangle (axis cs:2.32,0.0833333);
\path[draw=none,fill=histcolor!85] (axis cs:2.68,0.00007) rectangle (axis cs:3.32,0.276667);
\path[draw=none,fill=histcolor!85] (axis cs:3.68,0.00007) rectangle (axis cs:4.32,0.406667);
\path[draw=none,fill=histcolor!85] (axis cs:4.68,0.00007) rectangle (axis cs:5.32,0.183333);
\path[draw=none,fill=histcolor!85] (axis cs:5.68,0.00007) rectangle (axis cs:6.32,0.0366667);
\path[draw=none,fill=histcolor!85] (axis cs:6.68,0.00007) rectangle (axis cs:7.32,0.00333333);
\node[anchor=south,font=\scriptsize,text=histcolor,inner sep=1pt,yshift=2pt] at (axis cs:4,0.406667) {40.7\%};
\node[anchor=south west,font=\scriptsize,text=histcolor,inner sep=1pt,yshift=2pt] at (axis cs:7,0.00333333) {0.333\%};

